Deep Learning Aided Broadcast Codes with Feedback

Deep learning aided codes have been shown to improve code performance in feedback codes in high noise regimes due to the ability to leverage non-linearity in code design. In the additive white Gaussian broadcast channel (AWGN-BC), the addition of feedback may allow the capacity region to extend far beyond the capacity region of the channel without feedback, enabling higher data rates. On the other hand, there are limited deep-learning aided implementations of broadcast codes. In this work, we extend two classes of deep-learning assisted feedback codes to the AWGN-BC channel; the first being an RNN-based architecture and the second being a lightweight MLP-based architecture. Both codes are trained using a global model, and then they are trained using a more realistic vertical federated learning based framework. We first show that in most cases, using an AWGN-BC code outperforms a linear-based concatenated scheme. Second, we show in some regimes, the lightweight architecture far exceeds the RNN-based code, but in especially unreliable conditions, the RNN-based code dominates. The results show the promise of deep-learning aided broadcast codes in unreliable channels, and future research directions are discussed.

==> LightCodeBC.tex <==
We describe the encoding and decoding process for the LightCode-based scheme for Broadcast channels. Unlike GBAF and Robust Power-constrained coding, this scheme operates symbol by symbol reducing the number of required parameters. The encoder and both decoders consist of a \textit{feature extractor} followed by a multi-layer perceptron (MLP). We go over in detail the encoder and decoder architechure below.

\subsection{Encoding}
As mentioned, the encoding process its two fold. Encoding starts with a feature extractor module, followed by an MLP which outputs a symbol for transmission. This process is encapsulated by 
\begin{align*}
    x[t] = \alpha_t \phi\big(&W_1, W_2, z_1[t-1] z_1[t-2],\cdots, \\
    &z_1[1], z_2[t-1], z_2[t-2], \cdots, z_2[1]\big)
\end{align*}
 where $\alpha_t$ is the scaling factor that ensures the power constraint $\sum_{i=1}^D\alpha_i^2 = N$. That is, all the previous feedback and the messages for the two users is the input to the encoder, which in turn outputs a symbol for transmission $x[t]$. 

 \subsubsection{Feature Extractor}
 The feature extractor (FE) is designed as follows. The input of the feature extractor takes the message vectors $W_1, W_2$, the output of the MLP of the previous round $x[t-1]$, and the feedback from all previous rounds. Specifically, 
 \begin{align}
     \rvect[t] = \FE\big(&W_1, W_2, z_1[t-1] z_1[t-2],\cdots, \\
    &z_1[1], z_2[t-1], z_2[t-2], \cdots, z_2[1], x[t-1]\big) \nonumber
 \end{align}

The FE consists of multiple linear modules followed by ReLu units. (Insert Picture). 

\subsubsection{Encoder MLP} The FE is followed by a two layer MLP unit. The input of the encoder MLP takes the output of the FE and outputs a symbol $\Tilde{x}[t]$. Specifically, the input-output relationship of this is given by 
\begin{align}
    \Tilde{x}[t] = \MLP_2\paren{\rvect[t]}
\end{align}
where $\MLP_2\paren{\cdot}$ denotes the function of a two-layer MLP. 

\subsubsection{Power Normalization}
Finally, the output of the MLP is normalized so that the power constraint is obeyed specifically, we have that 
\begin{align}
    x[t] = w_t \lambda_t^{(J)}(\Tilde{x}[t])
\end{align}
where $w_t$ are trainable power weights such that $\sum_{t}w_t = N$ and $\lambda_t^{(J)}$ is a normalization function applied to $\Tilde{x}[t]$. 
\subsection{Decoding}
The decoding process is relatively similar to the encoding process, sans a power control layer. Just like the encoder, the decoder at each receiver consists of a FE layer and a single layer MLP. We briefly cover the input-output relationships of each layer. 
\subsubsection{Feature Extractor}
The architecture of the FE is nearly identical to that in the encoder. The decoder FE takes in all the $N$ received symbols and produces a feature vector $\rvect_d$. Specifically, the feature vector at the $k$th receiver is 
\begin{align*}
    \rvect_k = \FE\paren{\{y_k[t]\}_{t=0}^{N-1}}
\end{align*}


\subsubsection{Decoder MLP}
The decoder consists of a single layer MLP for classification. It takes as input the output of the FE and, in turn, returns a $2^{\lceil NR_k\rceil}$ vector. This vector serves as an indicator for the predicted message $W_k$. Specifically, the message $W_k$ corresponds to one entry in the $2^{\lceil NR_k\rceil}$-length output vector. The output of the MLP is given by 
\begin{align*}
    \dvect_k = \MLP\paren{\rvect_k}
\end{align*}

From this, the estimated message $\hat{W}_k$ is given by 
\begin{align}
    \hat{W}_k = f_{bin}\paren{\argmax \ \dvect_k }
\end{align}
where $f_{bin}(\cdot)$ maps the input to a binary representation.


\subsection{Model Training and Inference}

To Do: Model and training Details here. 





==> results.tex <==
In this section we simulate the proposed BC schemes and compare with the linear scheme and the single user scheme.  

\subsection{Performance with Feedback Noise}
Below, we compare the performance of the codes against varying feedback noise. For the two user broadcast scenarios, we set the blocklength $K$ per user to $6$ and set the number of channel uses $N$ to $18$. Thus, the rate per user is $R = 1/3$ and the sum rate is $R_{sum} =2/3$. To compare to the single user case, we halve the blocklength so that the single user rate is $R = 2/3$.  
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{AllSchemes.png}
    \caption{Code BLER as a function of feedback noise power}
    \label{fig:feedbacknoise}
\end{figure}

Observing Figure \ref{fig:feedbacknoise}, it can be seen that the linear coding scheme performs exceptionally well in the low feedback noise power scheme. As the feedback noise intensifies, the learned codes outperform due to being able to exploit non-linearity in coding. Further, it can be seen that there is a blocklength gain in the learned code when using a broadcast scheme versus time division. 

(Simulations currently running for BC light on henri)


(Simulations currently running for SU light on gilbreth)


\subsection{Perfect Feedback Case}
Here, we compare the performance of the codes with perfect feedback and varying forward SNR. 

\subsection{Power Control}

==> robustP.tex <==
Now we describe the encoding and decoding process for the power constrained scheme for broadcast channels. As mentioned before, there is a single encoder which consists of a set of $t$ functions $f_t(\cdot)$, for $t \in [N]$ which maps the messages $W_1,W_2$ and all of the feedback to a stream of $N$ symbols $x[1], \cdots, x[N]$ according to the power constraint in \eqref{eqn:powerCst}. However, this would require the design of $N$ encoder functions, which may become computationally demanding. Instead, define a single signal generation function $f$ such that the encoding process is given by 
\begin{align}
    x[t] = f(W_1, W_2, z_1[k-1], z_2[t-1], \svect[t])
\end{align}
where $\svect[k]$ is called the state vector which propagates over time through the state propagation function $h$ given by 
\begin{align}
    \svect[t] = h\paren{W_1,W_2,  z_1[t-1], z_2[t-1], \svect[t-1]}
\end{align}
In this way, the encoding model is a general non-linear extension of a state-space model for linear encoding \cite{kim2020deepcode}. Further, only $f$, $h$, and $g_1$, $g_2$ must be designed for the optimization problem in \eqref{eqn:optProblem} instead of $N$ unique encoding functions $f_t$. Unless otherwise stated, it is assumed all initial conditions are 0. That is, $z_k[-1] = 0$ and $\svect[-1] = 0$.  

\subsection{Encoding}
The encoding scheme consists of two gated recurrent units (GRUs), a non-linear layer, and a power control layer. We cover the purpose of each layer in the following. 
\subsubsection{GRU layer}
This layer consists of two layers of unidrectional GRUs in order to capture the time correlation of the feedback signals causally with the purpose of emanating the behavior of the function $h$. The network can be described as 
\begin{align}
    \svect_1[t] &= \GRU_1 \paren{W_1, W_2, z_1[t-1], z_2[t-1], \svect_1[t-1]}\\ 
    \svect_2[t] &= \GRU_2\paren{\svect_1[t], \svect_2[t-1]} 
\end{align}
where $\GRU_i$ denotes a GRU processing at layer $i$ and $\svect_i[t]$ is the resulting state vector by GRU $i$ at time $k$. Letting $\svect[t] = [\svect_1[t], \svect_2[t]]$, it follows that this layer performs the process 
\begin{align*}
    \svect[k] = h \paren{W_1, W_2, z_1[t-1], z_2[t-1], \svect[t-1]}
\end{align*}
where the GRUs perform the behavior of $h$. 

\subsubsection{Non-linear layer}
A non-linear layer follows the GRU layer. The process of the non-linear layer is given by 
\begin{align*}
    \Tilde{x}[t] = \phi(\textbf{w}_e^T \svect_2[t] + b_e)
\end{align*}
where $\textbf{w}_e$ and $b_e$ are the trainable weights and biases, respectively and $\phi$ is a hyperbolic tangent activation function. 

\subsection{Power Control Layer}
The power control layer is used to optimize the power distribution subject to the power constraint in \eqref{eqn:powerCst}. This layer consists of a normalization layer and a power-weight multiplication. The resulting signal is 
\begin{align}
    x[t] = w_t \lambda_t^(J)\paren{\Tilde{x}[t]}
\end{align} where $\lambda_t^(J)$ is a normalization function applied to $\Tilde{x}[t]$ and $w_t$ is a trainable power weight such that $\sum_{t=1}^N w_t^2 = N$. It is shown in Kim \textit{et al.} that this method of power control converges to the power constraint almost surely with large amounts of training data. 

\subsection{Decoding}
The decoding functions $g_k$ each consist of bi-directional GRUs, an attention layer, and a non-linear layer. The function of each layer is outlined below for each respective decoding function $g_k$.

\subsubsection{Bi-directional GRUs} Two layers of bi-directional GRUs are used to capture the forward and backward time correlation of the received signal. The input-output relationship of the forward direction GRUs are given by 
\begin{align*}
    \rvect_{f,1}[t] &=\GRU_{f,1}\paren{y[t], \rvect_{f,1}[t-1]},\\
    \rvect_{f,2}[t] &=\GRU_{f,2}\paren{\rvect_{f,1}[t], \rvect_{f,2}[t-1]},
\end{align*}
and the backward direction GRUs are given by
\begin{align*}
    \rvect_{b,1}[t] &=\GRU_{b,1}\paren{y[t], \rvect_{b,1}[t+1]},\\
    \rvect_{b,2}[t] &=\GRU_{b,2}\paren{\rvect_{b,1}[t], \rvect_{b,2}[t+1]},
\end{align*}
where $\GRU_{f,i}$ and $\GRU_{b,i}$ represent the GRU unit at layer $i$ in the forward and backward direction, respectively. 

\subsubsection{Attention Layer} The state vectors at the output of the GRUs are the input to the attention layer. The purpose of this layer is to enable to decoder to fully exploit the noisy signal information $\{y[t]\}_{t=1}^N$. The attention layer takes the structure
\begin{align*}
    \rvect_{f,att} = \sum_{t=1}^N \alpha_{f,t}\rvect_{f,2}[t], \ \rvect_{b,att} = \sum_{t=1}^N \alpha_{b,t}\rvect_{b,2}[t],
\end{align*}
where $\alpha_{f,t}$ and $\alpha_{b,t}$ are the rainable attention weights applied to the forward and backward state vectors, respectively. The two vectors are stacked to capture the forward and backward directional information separately as
\begin{align*}
    \rvect_{att} = [\rvect_{f,att}^T, \rvect_{b,att}^T]
\end{align*}

\subsubsection{Non-linear Layer} At the final stage of the decoder, a non-linear layer is used to obtain the estimate $\hat{W}_k$ by using the feature vector $\rvect_{att}$. This layer is described by 
\begin{align*}
    \hat{\dvect}=\theta\paren{\textbf{W}_d\rvect_{att} + \vvect_d}
\end{align*}

where $\theta$ is an activation function (softmax) and $\textbf{W}_d$ and $\vvect_d$ are the trainable weights and biases, respectively. We set the size of the output vector $\dvect$ as $2^K$; thus, $\hat{\dvect}$ denotes the probability distribution of $2^K$ messages. 

\subsection{Model Training and Inference}
For the single user case, the cross entropy (CE) loss $CE\paren{\dvect,\hat{\dvect}} = - \sum_{i=1}^{2^K}d_i \log \hat{d}_i$ where $\dvect \in \{0,1\}^{2^K}$ is the one-hot representation  of the message vector $W$.  For the inference, the largest entry of $\hat{\dvect}$ is forced to 1 and the rest 0. Since the entire bit stream is a block by using one-hot vectors, the optimization problem in \eqref{eqn:optProblem} is transformed into a classification problem. 

For the two user case, a similar procedure is followed. Instead, however, the loss is instead the sum of the cross entropy losses of each receiver. That is, the loss is given as 
\begin{align}
    L\paren{\dvect_1, \hat{\dvect}_1, \dvect_2, \hat{\dvect}_2} &= CE\paren{\dvect_1,\hat{\dvect_1}} + CE\paren{\dvect_2,\hat{\dvect_2}} 
\end{align}



